Vainu Bappu Memorial Lecture: What is a sunspot?

Sunspots have been known in the West since Galileo Galilei and Thomas Harriot first used telescopes to observe the Sun nearly four centuries ago; they have been known to the Chinese for more than two thousand years. They appear as relatively dark patches on the surface of the Sun, and are caused by concentrations of magnetism which impede the flow of heat from deep inside the Sun up to its othewise brilliant surface. The spots are not permanent: the total number of spots on the Sun varies cyclically in time, with a period of about eleven years, associated with which there appear to be variations in our climate. When there are many spots, it is more dangerous for spacecraft to operate. The cause of the spots is not well understood; nor is it known for sure how they die. Their structure beneath the surface of the Sun is in some dispute, although much is known about their properties at the surface, including an outward material flow which was discovered by John Evershed observing the Sun from Kodaikanal a hundred years ago. I shall give you a glimpse of how we are striving to deepen our understanding of these fascinating features, and of some of the phenomena that appear to be associated with them.

==> ascifile.tex <==
Vainu Bappu Memorial Lecture: What is a sunspot?

D. O. Gough

  Sunspots have been known in the West since Galileo Galilei and
  Thomas Harriot first used telescopes to observe the Sun nearly four
  centuries ago; they have been known to the Chinese for more than two
  thousand years.  They appear as relatively dark patches on the
  surface of the Sun, and are caused by concentrations of magnetism
  which impede the flow of heat from deep inside the Sun up to its
  othewise brilliant surface.  The spots are not permanent: the total
  number of spots on the Sun varies cyclically in time, with a period
  of about eleven years, associated with which there appear to be
  variations in our climate.  When there are many spots, it is more
  dangerous for spacecraft to operate.  The cause of the spots is not
  well understood; nor is it known for sure how they die.  Their
  structure beneath the surface of the Sun is in some dispute,
  although much is known about their properties at the surface,
  including an outward material flow which was discovered by John
  Evershed observing the Sun from Kodaikanal a hundred years ago.  I
  shall give you a glimpse of how we are striving to deepen our
  understanding of these fascinating features, and of some of the
  phenomena that appear to be associated with them.
